Bifurcations of Riemann Ellipsoids

We give an account of the various changes in the stability character in the five types of Riemann ellipsoids by establishing the occurrence of different quasi-periodic Hamiltonian bifurcations. Suitable symplectic changes of coordinates, that is, linear and non-linear normal form transformations are performed, leading to the characterisation of the bifurcations responsible of the stability changes. Specifically we find three types of bifurcations, namely, Hamiltonian pitchfork, saddle-centre and Hamiltonian-Hopf in the four-degree-of-freedom Hamiltonian system resulting after reducing out the symmetries of the problem. The approach is mainly analytical up to a point where non-degeneracy conditions have to be checked numerically. We also deal with the regimes in the parametric plane where Liapunov stability of the ellipsoids is accomplished. This strong stability behaviour occurs only in two of the five types of ellipsoids, at least deductible only from a linear analysis.

==> Extra_formula.tex <==

 	\bas
L&:=&	\left[ \begin {array}{cccccccc} 0&0&0&0&a&b&0&0
	\\ \noalign{\medskip}0&0&0&0&b&c&0&0\\ \noalign{\medskip}0
	&0&0&0&0&0&d&m\\ \noalign{\medskip}0&0&0&0&0&0&m&f\\ \noalign{\medskip}g&h&0&0&0&0&0&0
	\\ \noalign{\medskip}h&i&0&0&0&0&0&0
	\\ \noalign{\medskip}0&0&j&k&0&0&0&0
	\\ \noalign{\medskip}0&0&k&l&0&0&0&0\end {array}
	\right] 
	\eas 
 with the following entries:
	\bas
	a&:=&1-{\frac {{b_{{2}}}^{2}}{{b_{{1}}}^{4}{b_{{2}}}^{4}+{b_{{1}}}^{2}+{b_{
					{2}}}^{2}}},
				\\
		b&:=&		-{\frac {b_{{1}}b_{{2}}}{{b_{{1}}}^{4}{b_{{2}}}^{4}+{b_{{1}}}^{2}+{b_{
								{2}}}^{2}}},	
							\\
							c&:=&
							1-{\frac {{b_{{1}}}^{2}}{{b_{{1}}}^{4}{b_{{2}}}^{4}+{b_{{1}}}^{2}+{b_{
											{2}}}^{2}}},
\\
	d&:=& \frac{\sqrt{g \pi}}{\alpha} \left(-(b_1+b_2) f(b_1,b_2)\sqrt{t}+(b_1-b_2) f(-b_1,b_2)\sqrt{tt}\right),
	\\
	f&:=&  \frac{\sqrt{g \pi}}{\alpha} \left((b_1+b_2) f(b_1,b_2)\sqrt{t}+(b_1-b_2) f(-b_1,b_2)\sqrt{tt}\right),
	\\
	j&:=&  {\frac {\sqrt{g \pi} \left( {b_{{1}}}^{2}{b_{{2}}}^{4}-1 \right) ^{2}}{ \left( {b_
				{{1}}}^{4}{b_{{2}}}^{2}-1 \right) ^{2}}}
	\left((b_1+b_2) f(b_2,b_1)\sqrt{t}-(b_1-b_2) f(b_2,-b_1)\sqrt{tt}\right),
	\\
	l&:=&
	 {\frac {\sqrt{g \pi} \left( {b_{{1}}}^{2}{b_{{2}}}^{4}-1 \right) ^{2}}{ \left( {b_
				{{1}}}^{4}{b_{{2}}}^{2}-1 \right) ^{2}}}
	 \left(-(b_1+b_2) f(b_1,b_2)\sqrt{t}-(b_1-b_2) f(b_2,-b_1)\sqrt{tt}\right),
  \\m&:=&  \frac{k b_2}{b_1} \frac{\left( {b_
			{{1}}}^{4}{b_{{2}}}^{2}-1 \right)}{\left( {b_
			{{1}}}^{2}{b_{{2}}}^{4}-1 \right)},
   \\
   k&:=&
	\frac{2 b_1^4 b_2^3\sqrt{\zeta g 2 \pi}}{\sqrt {b_{{1}} \left( {b_{{1}}}^{2}{b_{{2}}}^{4}-1 \right)  \left( {b_
				{{1}}}^{4}{b_{{2}}}^{2}-1 \right) }}
	\eas
	
	

 \bas 
 h&:=&-8\,b_{{2}}g\pi\, \left( -2\,{b_{{1}}}^{6}{b_{{2}}}^{6} \left( {b_{{1}}}^{4}+{b_{{1}}}^{2}{b_{{
2}}}^{2}+{b_{{2}}}^{4} \right) +{b_{{1}}}^{2}{b_{{2}}}^{2} \left( {b_{
{1}}}^{2}+{b_{{2}}}^{2} \right)  \left( {b_{{1}}}^{8}{b_{{2}}}^{8}-{b_
{{1}}}^{4}+5\,{b_{{1}}}^{2}{b_{{2}}}^{2}-{b_{{2}}}^{4} \right) -8\,{b_
{{1}}}^{2}{b_{{2}}}^{2}+3\,{b_{{1}}}^{4}+3\,{b_{{2}}}^{4}
 \right)ee
\\
&+&
8\,b_{{2}}g\pi\, \left( b_{{1}}{b_{{2}}}^{2}-1 \right)  \left( b_{{1}}
{b_{{2}}}^{2}+1 \right)  \left( 2\,{b_{{1}}}^{8}{b_{{2}}}^{8}-2\,{b_{{
1}}}^{6}{b_{{2}}}^{4}-2\,{b_{{1}}}^{4}{b_{{2}}}^{6}-{b_{{1}}}^{4}+4\,{
b_{{1}}}^{2}{b_{{2}}}^{2}-{b_{{2}}}^{4} \right) ef
\\
&+&
8\,{\frac {{b_{{2}}}^{2}g\pi\, \left( {b_{{1}}}^{2}{b_{{2}}}^{2} \left( {b_{{1}}}^{6}{b_{{2}}}^{4}-3\,{b_{{1
}}}^{4}+{b_{{2}}}^{4} \right) +4\,{b_{{1}}}^{2}-3\,{b_{{2}}}^{2}
 \right)  \left( b_{{1}}^2-b_{{2}}^2 \right)   \sqrt { \left( {b_{{1}}}^{2}b_{{2}}-1 \right) 
 \left( {b_{{1}}}^{2}b_{{2}}+1 \right) }}{b_{{1}}}}
 \eas
\bas
h&:=&
\frac{-2\beta b_2(b_1^2-b_2^2)\sqrt{b_1^4b_2^2-1}}{b_1}\left(4 b_{1}^{2}-3 \left(b_{1}^{6}+1\right) b_{2}^{2}+b_{1}^{2} \left(b_{1}^{6}+1\right) b_{2}^{6}\right)
\\&&
+ \frac{-2\beta ee b_1}{b_1}\left(-b_{2}^{10} b_{1}^{6} \left(b_{1}^{6}+b_{1}^{4} b_{2}^{2}-2\right)+b_{2}^{6} b_{1}^{2} \left(2 b_{1}^{8}+2 b_{1}^{6} b_{2}^{2}-4 b_{1}^{2}+b_{2}^{2}\right)+b_{2}^{2} \left(b_{1}^{8}-4 b_{1}^{6} b_{2}^{2}+8 b_{1}^{2}-3 b_{2}^{2}\right)-3 b_{1}^{4}
\right)
\\&&
 \frac{-2\beta ef b_1(b_1^2b_2^4-1)
}{b_1}\left(2 b_{1}^{8} b_{2}^{8}-2 b_{1}^{6} b_{2}^{4}+4 b_{1}^{2} b_{2}^{2}-b_{2}^{4}-b_{1}^{4} \left(2 b_{2}^{6}+1\right)\right)
\eas
\bas
i&=&
\frac{-\beta}{b_2}\left(F(b_2,b_1)ee+G(b_2,b_1)ef\right)
\\&&
{-\beta(b_1^2-b_2^2)\sqrt{b_1^4b_2^2-1}}
\left(6 b_{1}^{8} b_{2}^{6}-9 b_{1}^{4} b_{2}^{4}+5 b_{2}^{2}+3 b_{1}^{2} \left(b_{2}^{6}-1\right)+b_{1}^{6} \left(-4 b_{2}^{8}+2 b_{2}^{2}\right)\right)
\eas
\bas
G:&=&\frac{- b_2}{b_1^2\beta}\left(b_1eeF(b_1,b_2)
+b_1({b_1}^2{b_2}^4-1)efG(b_1,b_2)\right)
\\&&-
\frac{ {b_2}^2}{b_1^2\beta}(b_1^2-b_2^2)\sqrt{({b_1}^4{b_2}^2-1)} 
\left(b_{1}^{6} b_{2}^{6} \left(7 b_{1}^{2}-5 b_{2}^{2}\right)-b_{1}^{2} b_{2}^{2} \left(5 b_{1}^{4}-b_{2}^{4}\right)+b_{1}^{2}+b_{2}^{2}\right).
\eas
Where 

	\bas
	\zeta&:=& -\left( {b_{{2}}}^{2}{b_{{1}}}^{2} \left( {b_{{1}}}^{4}{b_{{2}}}^{2}+{
		b_{{1}}}^{2}{b_{{2}}}^{4}+6 \right) + \left( {b_{{1}}}^{2}+{b_{{2}}}^{
		2} \right) ^{2} \right) {\it ee}\,\sqrt {{b_{{1}}}^{4}{b_{{2}}}^{2}-1}
	+2\,{b_{{2}}}^{2}{b_{{1}}}^{2} \left( {b_{{1}}}^{2}{b_{{2}}}^{4}-1
	\right) {\it ef}\,\sqrt {{b_{{1}}}^{4}{b_{{2}}}^{2}-1}
	\\&&
	-b_{{2}}
	\left( {b_{{1}}}^{2} \left( {b_{{1}}}^{2}+7\,{b_{{2}}}^{2} \right) +
	\left( {b_{{1}}}^{2}+{b_{{2}}}^{2} \right) ^{2} \right)  \left( {b_{{
				1}}}^{4}{b_{{2}}}^{2}-1 \right) 
\\
\beta&:=&\frac{4g\pi}{
 \left( b_{{1}}^2-b_{{2}}^2 \right) ^{2}\left( {b_{{1}}}^{4}{b_{{2}}}^{2}-1 \right) ^{\frac{3}{2}}
\left( {b_{{1}}}^{2}{b_{{2}}}^{4}-1 \right) ^{2}},
	\eas
	\bas
	\alpha&:=&\sqrt {b_{{1}}}\sqrt [4]{{b_{{1}}}^{4}{b_{{2}}}^{2}-1} \left( {b_{{1}}
	}^{2}{b_{{2}}}^{4}-1 \right) ^{5/2} \left( {b_{{1}}}^{2}-{b_{{2}}}^{2}
	\right) 
	\\
	f(b_1,b_2)&:=&{b_{{1}}}^{6}{b_{{2}}}^{6}-2\,{b_{{1}}}^{5}{b_{{2}}}^{7}+{b_{{1}}}^{4}
	{b_{{2}}}^{2}-2\,{b_{{1}}}^{3}{b_{{2}}}^{3}+3\,{b_{{1}}}^{2}{b_{{2}}}^
	{4}-1
\\
 F(b_1,b_2)&:=&{b_{{1}}}^{6}{b_{{2}}}^{6} \left( 3\,{b_{{1}}}^{6}{b_{{2}}}^{4}+{b_{{1
}}}^{4}{b_{{2}}}^{6}+2\,{b_{{1}}}^{4}-22\,{b_{{1}}}^{2}{b_{{2}}}^{2}+8
\,{b_{{2}}}^{4} \right) 
\\&&
-{b_{{2}}}^{4}-5\,{b_{{1}}}^{4}-{b_{{1}}}^{2}{
b_{{2}}}^{2} \left( 3\,{b_{{1}}}^{6}-20\,{b_{{1}}}^{4}{b_{{2}}}^{2}+4
\,{b_{{1}}}^{2}{b_{{2}}}^{4}+{b_{{2}}}^{6}-2 \right)
\\
G(b_1,b_2)&=&
{b_{{1}}}^{2}{b_{{2}}}^{2} \left( {b_{{1}}}^{8}{b_{{2}}}^{4}+3\,{b_{{1
}}}^{6}{b_{{2}}}^{6}-{b_{{1}}}^{6}-7\,{b_{{1}}}^{4}{b_{{2}}}^{2}-2
 \right) +{b_{{2}}}^{4}+5\,{b_{{1}}}^{4}
 \eas


==> fonts/ref.tex <==

@article{roberts1999symmetries,
	title={Symmetries of Riemann ellipsoids},
	author={Roberts, RM and Dias, MER Sousa},
	journal={Resenhas do Instituto de Matem{\'a}tica e Estat{\'\i}stica da Universidade de S{\~a}o Paulo},
	volume={4},
	number={2},
	pages={183--221},
	year={1999}
}
@article{broer2010kam,
	title={kam Theory: quasi-periodicity in dynamical systems},
	author={Broer, Henk W and Sevryuk, Mikhail B},
	journal={Handbook of Dynamical Systems},
	volume={3},
	number={C},
	pages={249--344},
	year={2010}
}
@book{meyer1999periodic,
	title={Periodic solutions of the N-body problem},
	author={Meyer, Kenneth R},
	volume={1719},
	year={1999},
	publisher={Springer Science \& Business Media}
}
@book{hanssmann2006local,
	title={Local and semi-local bifurcations in Hamiltonian dynamical systems: results and examples},
	author={Han{\ss}mann, Heinz},
	year={2006},
	publisher={Springer}
}

@article{broer2007quasi,
	title={The quasi-periodic Hamiltonian Hopf bifurcation},
	author={Broer, Henk W and Han{\ss}mann, Heinz and Hoo, Jun},
	journal={Nonlinearity},
	volume={20},
	number={2},
	pages={417},
	year={2007},
	publisher={IOP Publishing}
}

@article{meyer2017poincare,
	title={Poincar{\'e}’s Continuation Method},
	author={Meyer, Kenneth R and Offin, Daniel C},
	booktitle={Introduction to Hamiltonian Dynamical Systems and the N-Body Problem},
	pages={225--238},
	year={2017},
	publisher={Springer}
}
@article{fasso2014erratum,
	title={Erratum Erratum to: Stability Properties of the Riemann Ellipsoids},
	author={Fass{\`o}, Francesco and Lewis, Debra},
	journal={Archive for Rational Mechanics and Analysis},
	volume={212},
	number={3},
	pages={1065},
	year={2014},
	publisher={Springer Nature BV}
}
@article{gazor2019vector,
	title={Vector potential normal form classification for completely integrable solenoidal nilpotent singularities},
	author={Gazor, Majid and Mokhtari, Fahimeh and Sanders, Jan A},
	journal={Journal of Differential Equations},
	volume={267},
	number={1},
	pages={407--442},
	year={2019},
	publisher={Elsevier}
}
@article{golmakani2011lorenz,
	title={Lorenz attractors in unfoldings of homoclinic-flip bifurcations},
	author={Golmakani, A and Homburg, AJ},
	journal={Dynamical Systems},
	volume={26},
	number={1},
	pages={61--76},
	year={2011},
	publisher={Taylor \& Francis}
}
@article{homburg2014construction,
	title={Construction of codimension one homoclinic cycles},
	author={Homburg, Ale Jan and Kellner, Maria and Knobloch, J{\"u}rgen},
	journal={Dynamical Systems},
	volume={29},
	number={1},
	pages={133--151},
	year={2014},
	publisher={Taylor \& Francis}
}
@article{diekman2013derived,
	title={Derived patterns in binocular rivalry networks},
	author={Diekman, Casey O and Golubitsky, Martin and Wang, Yunjiao},
	journal={The Journal of Mathematical Neuroscience},
	volume={3},
	number={1},
	pages={1--23},
	year={2013},
	publisher={SpringerOpen}
}
@article{golubitsky2017homeostasis,
	title={Homeostasis, singularities, and networks},
	author={Golubitsky, Martin and Stewart, Ian},
	journal={Journal of mathematical biology},
	volume={74},
	number={1-2},
	pages={387--407},
	year={2017},
	publisher={Springer}
}
@article{tyson2003sniffers,
	title={Sniffers, buzzers, toggles and blinkers: dynamics of regulatory and signaling pathways in the cell},
	author={Tyson, John J and Chen, Katherine C and Novak, Bela},
	journal={Current opinion in cell biology},
	volume={15},
	number={2},
	pages={221--231},
	year={2003},
	publisher={Elsevier}
}
@article{alon2007network,
	title={Network motifs: theory and experimental approaches},
	author={Alon, Uri},
	journal={Nature Reviews Genetics},
	volume={8},
	number={6},
	pages={450--461},
	year={2007},
	publisher={Nature Publishing Group}
}
@article{xi2017synchronization,
	title={Synchronization of cyclic power grids: Equilibria and stability of the synchronous state},
	author={Xi, Kaihua and Dubbeldam, Johan LA and Lin, Hai Xiang},
	journal={Chaos: an interdisciplinary journal of nonlinear science},
	volume={27},
	number={1},
	pages={013109},
	year={2017},
	publisher={AIP Publishing LLC}
}
@inproceedings{van2018triadic,
	title={Triadic split-merge sampler},
	author={van Rossum, Anne C and Lin, Hai Xiang and Dubbeldam, Johan and van der Herik, H Jaap},
	booktitle={Tenth International Conference on Machine Vision (ICMV 2017)},
	volume={10696},
	pages={1069623},
	year={2018},
	organization={International Society for Optics and Photonics}
}
@article{xi2018power,
	title={Power-imbalance allocation control of power systems-secondary frequency control},
	author={Xi, Kaihua and Dubbeldam, Johan LA and Lin, Hai Xiang and van Schuppen, Jan H},
	journal={Automatica},
	volume={92},
	pages={72--85},
	year={2018},
	publisher={Elsevier}
}
@article{kooij2020kemeny,
	title={Kemeny’s constant for several families of graphs and real-world networks},
	author={Kooij, Robert E and Dubbeldam, Johan LA},
	journal={Discrete Applied Mathematics},
	volume={285},
	pages={96--107},
	year={2020},
	publisher={Elsevier}
}
@article{maria2006homogeneous,
	title={Homogeneous three-cell networks},
	author={Maria da Concei{\c{c}}ao, A Leite and Golubitsky, Martin},
	journal={Nonlinearity},
	volume={19},
	number={10},
	pages={2313},
	year={2006},
	publisher={IOP Publishing}
}
@article{golubitsky2004some,
	title={Some curious phenomena in coupled cell networks},
	author={Golubitsky, Martin and Nicol, Matthew and Stewart, Ian},
	journal={Journal of Nonlinear Science},
	volume={14},
	number={2},
	pages={207--236},
	year={2004},
	publisher={Springer}
}
@article{golubitsky2009bifurcations,
	title={Bifurcations from synchrony in homogeneous networks: linear theory},
	author={Golubitsky, Martin and Lauterbach, Reiner},
	journal={SIAM Journal on Applied Dynamical Systems},
	volume={8},
	number={1},
	pages={40--75},
	year={2009},
	publisher={SIAM}
}
@article{elmhirst2006nilpotent,
	title={Nilpotent Hopf bifurcations in coupled cell systems},
	author={Elmhirst, Toby and Golubitsky, Martin},
	journal={SIAM Journal on Applied Dynamical Systems},
	volume={5},
	number={2},
	pages={205--251},
	year={2006},
	publisher={SIAM}
}
@book{pikovsky2003synchronization,
	title={Synchronization: a universal concept in nonlinear sciences},
	author={Pikovsky, Arkady and Kurths, Jurgen and Rosenblum, Michael and Kurths, J{\"u}rgen},
	number={12},
	year={2003},
	publisher={Cambridge university press}
}

@article{arnold1972lectures,
	title={Lectures on bifurcations in versal families},
	author={Arnold, Vladimir I},
	booktitle={Vladimir I. Arnold-Collected Works},
	pages={271--340},
	year={1972},
	publisher={Springer}
}
@article{arnold1971matrices,
	title={On matrices depending on parameters},
	author={Arnold, Vladimir I},
	journal={Russian Mathematical Surveys},
	volume={26},
	number={2},
	pages={29},
	year={1971},
	publisher={IOP Publishing}
}
@article{stewart2003symmetry,
	title={Symmetry groupoids and patterns of synchrony in coupled cell networks},
	author={Stewart, Ian and Golubitsky, Martin and Pivato, Marcus},
	journal={SIAM Journal on Applied Dynamical Systems},
	volume={2},
	number={4},
	pages={609--646},
	year={2003},
	publisher={SIAM}
}
@article{golubitsky2005patterns,
	title={Patterns of synchrony in coupled cell networks with multiple arrows},
	author={Golubitsky, Martin and Stewart, Ian and T{\"o}r{\"o}k, Andrei},
	journal={SIAM Journal on Applied Dynamical Systems},
	volume={4},
	number={1},
	pages={78--100},
	year={2005},
	publisher={SIAM}
}
@article{golubitsky2006nonlinear,
	title={Nonlinear dynamics of networks: the groupoid formalism},
	author={Golubitsky, Martin and Stewart, Ian},
	journal={Bulletin of the american mathematical society},
	volume={43},
	number={3},
	pages={305--364},
	year={2006}
}

@article{stewart2004networking,
	title={Networking opportunity},
	author={Stewart, Ian},
	journal={Nature},
	volume={427},
	number={6975},
	pages={601--604},
	year={2004},
	publisher={Nature Publishing Group}
}
@article{golubitsky2004some,
	title={Some curious phenomena in coupled cell networks},
	author={Golubitsky, Martin and Nicol, Matthew and Stewart, Ian},
	journal={Journal of Nonlinear Science},
	volume={14},
	number={2},
	pages={207--236},
	year={2004},
	publisher={Springer}
}
@article{field2004combinatorial,
	title={Combinatorial dynamics},
	author={Field, Michael},
	journal={DYNAMICAL SYSTEMS-AN INTERNATIONAL JOURNAL},
	volume={19},
	number={3},
	pages={217--243},
	year={2004},
	publisher={TAYLOR \& FRANCIS LTD 2-4 PARK SQUARE, MILTON PARK, ABINGDON OR14 4RN, OXON~…}
}
@misc{MS2021,
	title={The {L}ie algebraic structure of colored network {L}ie algebras},
	author={Mokhtari, Fahimeh and Sanders, Jan A},
	year={2021}
}
@misc{homburg2010homoclinic,
	title={Homoclinic and Heteroclinic Bifurcations in Vector Fields, Handbook of Dynamical Systems, Vol. 3},
	author={Homburg, AJ and Sandstede, B},
	year={2010},
	publisher={North Holland, Amsterdam}
}
@article{ashwin1999heteroclinic,
	title={Heteroclinic networks in coupled cell systems},
	author={Ashwin, Peter and Field, Michael},
	journal={Archive for Rational Mechanics and Analysis},
	volume={148},
	number={2},
	pages={107--143},
	year={1999},
	publisher={Springer}
}
@article{sanders2003normal,
	title={Normal form theory and spectral sequences},
	author={Sanders, Jan A},
	journal={Journal of Differential Equations},
	volume={192},
	number={2},
	pages={536--552},
	year={2003},
	publisher={Elsevier}
}
@article{rink2013amplified,
	title={Amplified {H}opf bifurcations in feed-forward networks},
	author={Rink, Bob W and Sanders, Jan A},
	journal={SIAM Journal on Applied Dynamical Systems},
	volume={12},
	number={2},
	pages={1135--1157},
	year={2013},
	publisher={SIAM}
}

@article{nijholt2020quiver,
	title={Quiver representations and dimension reduction in dynamical systems},
	author={Nijholt, Eddie and Rink, Bob W and Schwenker, Sören},
	journal={SIAM Journal on Applied Dynamical Systems},
	volume={19},
	number={4},
	pages={2428--2468},
	year={2020},
	publisher={SIAM}
}
@article{golubitsky2006nonlinear,
	title={Nonlinear dynamics of networks: the groupoid formalism},
	author={Golubitsky, Martin and Stewart, Ian},
	journal={Bulletin of the american mathematical society},
	volume={43},
	number={3},
	pages={305--364},
	year={2006}
}
@article{golubitsky2009bifurcations,
	title={Bifurcations from synchrony in homogeneous networks: linear theory},
	author={Golubitsky, Martin and Lauterbach, Reiner},
	journal={SIAM Journal on Applied Dynamical Systems},
	volume={8},
	number={1},
	pages={40--75},
	year={2009},
	publisher={SIAM}
}

@article{maria2006homogeneous,
	title={Homogeneous three-cell networks},
	author={Maria da Concei{\c{c}}ao, A Leite and Golubitsky, Martin},
	journal={Nonlinearity},
	volume={19},
	number={10},
	pages={2313},
	year={2006},
	publisher={IOP Publishing}
}
@article{golubitsky2004some,
	title={Some curious phenomena in coupled cell networks},
	author={Golubitsky, Martin and Nicol, Matthew and Stewart, Ian},
	journal={Journal of Nonlinear Science},
	volume={14},
	number={2},
	pages={207--236},
	year={2004},
	publisher={Springer}
}
@article{gandhi2020bifurcations,
	title={Bifurcations on fully inhomogeneous networks},
	author={Gandhi, Punit and Golubitsky, Martin and Postlethwaite, Claire and Stewart, Ian and Wang, Yangyang},
	journal={SIAM Journal on Applied Dynamical Systems},
	volume={19},
	number={1},
	pages={366--411},
	year={2020},
	publisher={SIAM}
}
@incollection{karabacak2008heteroclinic,
    AUTHOR = {Ashwin, Peter and Karabacak, \"{O}zkan},
     TITLE = {Robust heteroclinic behaviour, synchronization, and ratcheting
              of coupled oscillators},
 BOOKTITLE = {Dynamics, games and science. {II}},
    SERIES = {Springer Proc. Math.},
    VOLUME = {2},
     PAGES = {125--140},
 PUBLISHER = {Springer, Heidelberg},
      YEAR = {2011},
   MRCLASS = {37C29 (34C15 34D06)},
  MRNUMBER = {2883274},
       DOI = {10.1007/978-3-642-14788-3\_10},
       URL = {https://doi-org.vu-nl.idm.oclc.org/10.1007/978-3-642-14788-3_10},
}
		
@article{aguiar2011dynamics,
	title={Dynamics of coupled cell networks: synchrony, heteroclinic cycles and inflation},
	author={Aguiar, M and Ashwin, Peter and Dias, A and Field, Michael},
	journal={Journal of nonlinear science},
	volume={21},
	number={2},
	pages={271--323},
	year={2011},
	publisher={Springer}
}
@incollection {MR2185000, AUTHOR = {Golubitsky, Martin and Stewart, Ian}, TITLE = {Synchrony versus symmetry in coupled cells}, BOOKTITLE = {E{QUADIFF} 2003}, PAGES = {13--24}, PUBLISHER = {World Sci. Publ., Hackensack, NJ}, YEAR = {2005}, MRCLASS = {37C10 (34C14 34C15 37C80)}, MRNUMBER = {2185000}, DOI = {10.1142/9789812702067\_0002}, URL = {https://doi-org.vu-nl.idm.oclc.org/10.1142/9789812702067_0002}, }
@article {MR2823037,
	AUTHOR = {Cagliero, Leandro and Szechtman, Fernando},
	TITLE = {Jordan-{C}hevalley decomposition in finite dimensional {L}ie
	algebras},
	JOURNAL = {Proc. Amer. Math. Soc.},
	FJOURNAL = {Proceedings of the American Mathematical Society},
	VOLUME = {139},
	YEAR = {2011},
	NUMBER = {11},
	PAGES = {3909--3913},
	ISSN = {0002-9939},
	MRCLASS = {17B20},
	MRNUMBER = {2823037},
	MRREVIEWER = {Mohammad Hailat},
	DOI = {10.1090/S0002-9939-2011-10827-X},
	URL = {https://doi-org.vu-nl.idm.oclc.org/10.1090/S0002-9939-2011-10827-X},
}
@book {MR1606831,
	AUTHOR = {Goodman, Roe and Wallach, Nolan R.},
	TITLE = {Representations and invariants of the classical groups},
	SERIES = {Encyclopedia of Mathematics and its Applications},
	VOLUME = {68},
	PUBLISHER = {Cambridge University Press, Cambridge},
	YEAR = {1998},
	PAGES = {xvi+685},
	ISBN = {0-521-58273-3; 0-521-66348-2},
	MRCLASS = {20G05 (14L35 14M17 17B10 20C30 20G20 22E46)},
	MRNUMBER = {1606831},
	MRREVIEWER = {James E. Humphreys},
}
@article {MR4183886,
	AUTHOR = {DeVille, Lee and Nijholt, Eddie},
	TITLE = {Circulant type formulas for the eigenvalues of linear network
	maps},
	JOURNAL = {Linear Algebra Appl.},
	FJOURNAL = {Linear Algebra and its Applications},
	VOLUME = {610},
	YEAR = {2021},
	PAGES = {379--439},
	ISSN = {0024-3795},
	MRCLASS = {05C50 (15A18 15B05 37E25)},
	MRNUMBER = {4183886},
	DOI = {10.1016/j.laa.2020.09.023},
	URL = {https://doi-org.vu-nl.idm.oclc.org/10.1016/j.laa.2020.09.023},
}


@article {MR4169252,
	AUTHOR = {Nijholt, Eddie and Rink, Bob W. and Schwenker, S\"{o}ren},
	TITLE = {Quiver representations and dimension reduction in dynamical
	systems},
	JOURNAL = {SIAM J. Appl. Dyn. Syst.},
	FJOURNAL = {SIAM Journal on Applied Dynamical Systems},
	VOLUME = {19},
	YEAR = {2020},
	NUMBER = {4},
	PAGES = {2428--2468},
	MRCLASS = {37C81 (16G20 34C14 34C45)},
	MRNUMBER = {4169252},
	DOI = {10.1137/20M1345670},
	URL = {https://doi-org.vu-nl.idm.oclc.org/10.1137/20M1345670},
}


@article {MR3908319,
	AUTHOR = {Nijholt, Eddie and Rink, Bob and Sanders, Jan},
	TITLE = {Center manifolds of coupled cell networks},
	JOURNAL = {SIAM Rev.},
	FJOURNAL = {SIAM Review},
	VOLUME = {61},
	YEAR = {2019},
	NUMBER = {1},
	PAGES = {121--155},
	ISSN = {0036-1445},
	MRCLASS = {37G10 (20M30 34C23 37G40)},
	MRNUMBER = {3908319},
	MRREVIEWER = {C\'{e}lia Sofia Moreira},
	DOI = {10.1137/18M1219977},
	URL = {https://doi-org.vu-nl.idm.oclc.org/10.1137/18M1219977},
}

@article{gu2018homogeneous,
	title={From homogeneous to heterogeneous network alignment via colored graphlets},
	author={Gu, Shawn and Johnson, John and Faisal, Fazle E and Milenkovi{\'c}, Tijana},
	journal={Scientific reports},
	volume={8},
	number={1},
	pages={1--16},
	year={2018},
	publisher={Nature Publishing Group}
}
@article {MR3059183,
	AUTHOR = {Thompson, G. and Wick, Z.},
	TITLE = {Subalgebras of {${\mathfrak{gl}}(3,\Bbb R)$}},
	JOURNAL = {Extracta Math.},
	FJOURNAL = {Extracta Mathematicae},
	VOLUME = {27},
	YEAR = {2012},
	NUMBER = {2},
	PAGES = {201--230},
	ISSN = {0213-8743},
	MRCLASS = {17B05 (22E60)},
	MRNUMBER = {3059183},
	MRREVIEWER = {K. Strambach},
}
@article {MR4059374,
	AUTHOR = {Gandhi, Punit and Golubitsky, Martin and Postlethwaite, Claire
	and Stewart, Ian and Wang, Yangyang},
	TITLE = {Bifurcations on fully inhomogeneous networks},
	JOURNAL = {SIAM J. Appl. Dyn. Syst.},
	FJOURNAL = {SIAM Journal on Applied Dynamical Systems},
	VOLUME = {19},
	YEAR = {2020},
	NUMBER = {1},
	PAGES = {366--411},
	MRCLASS = {34C23 (37G05 37G15)},
	MRNUMBER = {4059374},
	DOI = {10.1137/18M1230736},
	URL = {https://doi-org.vu-nl.idm.oclc.org/10.1137/18M1230736},
}
@article {MR3606590,
	AUTHOR = {Golubitsky, Martin and Stewart, Ian},
	TITLE = {Coordinate changes for network dynamics},
	JOURNAL = {Dyn. Syst.},
	FJOURNAL = {Dynamical Systems. An International Journal},
	VOLUME = {32},
	YEAR = {2017},
	NUMBER = {1},
	PAGES = {80--116},
	ISSN = {1468-9367},
	MRCLASS = {37C15 (34C20)},
	MRNUMBER = {3606590},
	MRREVIEWER = {Alexandre Artur Pinho Rodrigues},
	DOI = {10.1080/14689367.2016.1235136},
	URL = {https://doi-org.vu-nl.idm.oclc.org/10.1080/14689367.2016.1235136},
}
@book {MR1453120,
	AUTHOR = {Sharpe, R. W.},
	TITLE = {Differential geometry},
	SERIES = {Graduate Texts in Mathematics},
	VOLUME = {166},
	NOTE = {Cartan's generalization of Klein's Erlangen program,
	With a foreword by S. S. Chern},
	PUBLISHER = {Springer-Verlag, New York},
	YEAR = {1997},
	PAGES = {xx+421},
	ISBN = {0-387-94732-9},
	MRCLASS = {53Cxx (53-02)},
	MRNUMBER = {1453120},
	MRREVIEWER = {William Goldman},
}
@book {MR1251060,
	AUTHOR = {Collingwood, David H. and McGovern, William M.},
	TITLE = {Nilpotent orbits in semisimple {L}ie algebras},
	SERIES = {Van Nostrand Reinhold Mathematics Series},
	PUBLISHER = {Van Nostrand Reinhold Co., New York},
	YEAR = {1993},
	PAGES = {xiv+186},
	ISBN = {0-534-18834-6},
	MRCLASS = {17-02 (17B20 17B25 22E60)},
	MRNUMBER = {1251060},
	MRREVIEWER = {Stephen Slebarski},
}
@article{cushman1983normal,
	title={Normal form and representation theory},
	author={Cushman, Richard and Deprit, Andr{\'e} and Mosak, Richard},
	journal={Journal of mathematical physics},
	volume={24},
	number={8},
	pages={2102--2117},
	year={1983},
	publisher={AIP}
}
@book{HirschSmale1974,
	title={Differential equations, dynamical systems, and linear algebra},
	author={Hirsch, Morris W and Smale, Stephen},
	year={1974},
	publisher={Academic press}
}
@article{rink2015coupled,
	title={Coupled cell networks: semigroups, {L}ie algebras and normal forms},
	author={Rink, Bob and Sanders, Jan},
	journal={Transactions of the American Mathematical Society},
	volume={367},
	number={5},
	pages={3509--3548},
	year={2015}
}
@article{levelt1993semi,
	title={The semi-simple part of a matrix},
	author={Levelt, AHM},
	journal={Algoritmen In De Algebra (Aida), Nijmegen, August 1993},
	pages={83-86},
	year={1993},
	publisher={Citeseer}
}
@article {MR3953028,
	AUTHOR = {Mokhtari, Fahimeh and Sanders, Jan A.},
	TITLE = {Versal normal form for nonsemisimple singularities},
	JOURNAL = {J. Differential Equations},
	FJOURNAL = {Journal of Differential Equations},
	VOLUME = {267},
	YEAR = {2019},
	NUMBER = {5},
	PAGES = {3083--3113},
	ISSN = {0022-0396},
	MRCLASS = {34C20 (37G05)},
	MRNUMBER = {3953028},
	MRREVIEWER = {Majid Gazor},
	DOI = {10.1016/j.jde.2019.03.039},
	URL = {https://doi-org.vu-nl.idm.oclc.org/10.1016/j.jde.2019.03.039},
}
@article{mokhtari2018versal,
	title={Versal Normal Form for Nonsemisimple Singularities},
	author={Mokhtari, Fahimeh and Sanders, Jan A.},
	journal={arXiv preprint arXiv:1808.02690},
	year={2018}
}


@article{gazormokhtari2014normal,
	title={Normal forms of {H}opf-zero singularity},
	author={Gazor, Majid and Mokhtari, Fahimeh},
	journal={Nonlinearity},
	volume={28},
	number={2},
	pages={311},
	year={2014},
	publisher={IOP Publishing}
}

@book{berhuy2010introduction,
	title={An introduction to Galois cohomology and its applications},
	author={Berhuy, Gr{\'e}gory},
	volume={377},
	year={2010},
	publisher={Cambridge University Press}
}
@Book{            MR0323842,
	author        = {Humphreys, J.},
	address       = {New York},
	year          = {1972},
	publisher     = {Springer-Verlag},
	title         = {Introduction to {L}ie {A}lgebras and {R}epresentation
	{T}heory}
}
@article {MR0161898,
	AUTHOR = {Gerstenhaber, M.},
	TITLE = {The cohomology structure of an associative ring},
	JOURNAL = {Ann. of Math. (2)},
	FJOURNAL = {Annals of Mathematics. Second Series},
	VOLUME = {78},
	YEAR = {1963},
	PAGES = {267--288},
	ISSN = {0003-486X},
	MRCLASS = {16.90 (18.00)},
	MRNUMBER = {MR0161898 (28 \#5102)},
	MRREVIEWER = {M. Auslander},
}
@article{cushman56nilpotent,
	title={Nilpotent normal forms and representation theory of $\mathfrak{sl}_2(\mathbb{R})$, in ‘‘{M}ultiparameter {B}ifurcation {T}heory’’ ({M}. {G}olubitsky and {J}. {G}uckenheimer, {E}ds.)},
	author={Cushman, R.H. and Sanders, J.},
	journal={Contemporary Mathematics},
	volume={56},
	year={1986},
	pages={353--371}
}
@article{baider1992further,
	title={Further reduction of the {T}akens-{B}ogdanov normal form},
	author={Baider, A. and Sanders, J.A.},
	journal={Journal of Differential Equations},
	volume={99},
	number={2},
	pages={205--244},
	year={1992},
	publisher={Elsevier}
}
@misc{lewisfermat,
	title={Fermat User Guide},
	author={Lewis, R.H.}
}
@misc{lewis2008computer,
	title={Computer algebra system {F}ermat},
	author={Lewis, R.H.},
	year={2008}
}
@article{baez2014𝐺2,
	title={$\mathsf{G}_2$ and the rolling ball},
	author={Baez, J. and Huerta, J.},
	journal={Transactions of the American Mathematical Society},
	volume={366},
	number={10},
	pages={5257--5293},
	year={2014}
}
@article{Form00,
	title={{FORM} version 4.0},
	author={Kuipers, J. and Ueda, T. and Vermaseren, J.A.M. and Vollinga, J.},
	journal={Computer Physics Communications},
	volume={184},
	number={5},
	pages={1453--1467},
	year={2013},
	publisher={Elsevier}
}
@book {SVM2007,
	AUTHOR = {Sanders, J. A. and Verhulst, F. and Murdock, J.},
	TITLE = {Averaging {M}ethods in {N}onlinear {D}ynamical {S}ystems},
	SERIES = {Applied Mathematical Sciences},
	VOLUME = {59},
	EDITION = {Second},
	PUBLISHER = {Springer},
	ADDRESS = {New York},
	YEAR = {2007},
	PAGES = {xxii+431},
	ISBN = {978-0-387-48916-2; 0-387-48916-9},
	MRCLASS = {34-02 (34C29 34D15 34E10 34E15 37D10 37J40)},
	MRNUMBER = {MR2316999 (2008h:34001)},
	MRREVIEWER = {Zvi Artstein},
}
@article{mailybaev2001transformation,
	title={Transformation to versal deformations of matrices},
	author={Mailybaev, A.A.},
	journal={Linear Algebra and its Applications},
	volume={337},
	number={1-3},
	pages={87--108},
	year={2001},
	publisher={Elsevier}
}
@article{koccak1984normal,
	title={Normal forms and versal deformations of linear Hamiltonian systems},
	author={Ko{\c{c}}ak, H.},
	journal={Journal of Differential Equations},
	volume={51},
	number={3},
	pages={359--407},
	year={1984},
	publisher={Elsevier}
}
@article{knibbeler2017higher,
	title={Higher-dimensional automorphic {L}ie algebras},
	author={Knibbeler, Vincent and Lombardo, Sara and Sanders, Jan A},
	journal={Foundations of Computational Mathematics},
	volume={17},
	number={4},
	pages={987--1035},
	year={2017},
	publisher={Springer}
}


@article{kulkarni1980sigurdur,
	title={Sigurdur {H}elgason, {D}ifferential geometry, {L}ie groups and symmetric spaces},
	author={Kulkarni, Ravi S and others},
	journal={Bulletin (New Series) of the American Mathematical Society},
	volume={2},
	number={3},
	pages={468--476},
	year={1980},
	publisher={American Mathematical Society}
}

@article{anderson2015non,
	title={Non-Isomorphic Real Simple {L}ie Algebras of the Same Complex Type and Character},
	author={Anderson, Ian M},
	year={2015}
}

@book{knapp2013lie,
	title={Lie groups beyond an introduction},
	author={Knapp, Anthony W},
	volume={140},
	year={2013},
	publisher={Springer Science \& Business Media}
}

@article{cushman1986versal,
	title={Versal normal form at the {L}agrange equilibrium ${L}_4$},
	author={Cushman, R.H. and Kelley, A. and Ko{\c{c}}ak, H.},
	journal={Journal of Differential Equations},
	volume={64},
	number={3},
	pages={340--374},
	year={1986},
	publisher={Elsevier}
}

@article{sanders1994versal,
	title={Versal normal form computations and representation theory},
	author={Sanders, J.A.},
	journal={Computer Algebra and Differential Equations’, Cambrige University Press, Cambrige},
	pages={185--210},
	year={1994}
}

@article{springer1966some,
	title={Some arithmetical results on semi-simple {L}ie algebras},
	author={Springer, Tonny A},
	journal={Publications Math{\'e}matiques de l'IH{\'E}S},
	volume={30},
	pages={115--141},
	year={1966}
}
@article{kostant1956principal,
	title={THE PRINCIPAL THREE-DIMENSIONAL SUBGROUP AND THE BETTI NUMBERS OF A COMPLEX SIMPLE LIE GROUP.},
	author={Kostant, Bertram},
	journal={Bull. Soc. Math. France},
	volume={84},
	pages={251--281},
	year={1956},
	publisher={JSTOR}
}
@article{kostant1963lie,
	title={Lie group representations on polynomial rings},
	author={Kostant, Bertram},
	journal={American Journal of Mathematics},
	volume={85},
	number={3},
	pages={327--404},
	year={1963},
	publisher={JSTOR}
}
@book {MR1890629,
	AUTHOR = {Bourbaki, Nicolas},
	TITLE = {Lie groups and {L}ie algebras. {C}hapters 4--6},
	SERIES = {Elements of Mathematics (Berlin)},
	NOTE = {Translated from the 1968 French original by Andrew Pressley},
	PUBLISHER = {Springer-Verlag},
	ADDRESS = {Berlin},
	YEAR = {2002},
	PAGES = {xii+300},
	ISBN = {3-540-42650-7},
	MRCLASS = {17-01 (00A05 20E42 20F55 22-01)},
	MRNUMBER = {1890629 (2003a:17001)},
}
@unpublished {KLS15c,
	AUTHOR = {Knibbeler, V. and Lombardo, S. and Sanders, J. A.},
	TITLE = {Automorphic {L}ie {A}lgebras and {C}ohomology of {R}oot {S}ystems},
	NOTE = {arXiv:1512.07020  [math-ph]},
	YEAR = {2015}
}




@article{golubitsky2017coordinate,
	title={Coordinate changes for network dynamics},
	author={Golubitsky, Martin and Stewart, Ian},
	journal={Dynamical Systems},
	volume={32},
	number={1},
	pages={80--116},
	year={2017},
	publisher={Taylor \& Francis}
}

@article{aguiar2017patterns,
	title={Patterns of synchrony for feed-forward and auto-regulation feed-forward neural networks},
	author={Aguiar, Manuela AD and Dias, Ana Paula S and Ferreira, Flora},
	journal={Chaos: An Interdisciplinary Journal of Nonlinear Science},
	volume={27},
	number={1},
	pages={013103},
	year={2017},
	publisher={AIP Publishing LLC}
}
@article{aguiar2014lattice,
	title={The lattice of synchrony subspaces of a coupled cell network: Characterization and computation algorithm},
	author={Aguiar, Manuela AD and Dias, Ana Paula S},
	journal={Journal of Nonlinear Science},
	volume={24},
	number={6},
	pages={949--996},
	year={2014},
	publisher={Springer}
}
@article{algaba2019nonlinear,
	title={A nonlinear time transformation method to compute all the coefficients for the homoclinic bifurcation in the quadratic Takens--Bogdanov normal form},
	author={Algaba, Antonio and Chung, Kwok-Wai and Qin, Bo-Wei and Rodr{\'\i}guez-Luis, Alejandro J},
	journal={Nonlinear Dynamics},
	volume={97},
	number={2},
	pages={979--990},
	year={2019},
	publisher={Springer}
}

@article{algaba2016takens,
	title={Takens--Bogdanov bifurcations of equilibria and periodic orbits in the Lorenz system},
	author={Algaba, A and Dom{\'\i}nguez-Moreno, MC and Merino, M and Rodr{\'\i}guez-Luis, AJ},
	journal={Communications in Nonlinear Science and Numerical Simulation},
	volume={30},
	number={1-3},
	pages={328--343},
	year={2016},
	publisher={Elsevier}
}

@article{algaba1999takens,
	title={On the Takens-Bogdanov bifurcation in the Chua's equation},
	author={Algaba, Antonio and Freire, Emilio and Gamero, Estanislao and Rodriguez-Luis, Alejandro J},
	journal={IEICE Transactions on Fundamentals of Electronics, Communications and Computer Sciences},
	volume={82},
	number={9},
	pages={1722--1728},
	year={1999},
	publisher={The Institute of Electronics, Information and Communication Engineers}
}
@article{kang1998bifurcation,
	title={Bifurcation and normal form of nonlinear control systems, Part I},
	author={Kang, Wei},
	journal={SIAM Journal on Control and Optimization},
	volume={36},
	number={1},
	pages={193--212},
	year={1998},
	publisher={SIAM}
}
@article{pietras2019exact,
	title={Exact firing rate model reveals the differential effects of chemical versus electrical synapses in spiking networks},
	author={Pietras, Bastian and Devalle, Federico and Roxin, Alex and Daffertshofer, Andreas and Montbri{\'o}, Ernest},
	journal={Physical Review E},
	volume={100},
	number={4},
	pages={042412},
	year={2019},
	publisher={APS}
}

@article{pietras2019network,
	title={Network dynamics of coupled oscillators and phase reduction techniques},
	author={Pietras, Bastian and Daffertshofer, Andreas},
	journal={Physics Reports},
	volume={819},
	pages={1--105},
	year={2019},
	publisher={Elsevier}
}
@article{roberts1999symmetries,
	title={Symmetries of Riemann ellipsoids},
	author={Roberts, RM and Dias, MER Sousa},
	journal={Resenhas do Instituto de Matem{\'a}tica e Estat{\'\i}stica da Universidade de S{\~a}o Paulo},
	volume={4},
	number={2},
	pages={183--221},
	year={1999}
}
@article{fasso2014erratum,
	title={Erratum Erratum to: Stability Properties of the Riemann Ellipsoids},
	author={Fass{\`o}, Francesco and Lewis, Debra},
	journal={Archive for Rational Mechanics and Analysis},
	volume={212},
	number={3},
	pages={1065},
	year={2014},
	publisher={Springer Nature BV}
}
@article{roberts1999symmetries,
	title={Symmetries of Riemann ellipsoids},
	author={Roberts, RM and Dias, MER Sousa},
	journal={Resenhas do Instituto de Matem{\'a}tica e Estat{\'\i}stica da Universidade de S{\~a}o Paulo},
	volume={4},
	number={2},
	pages={183--221},
	year={1999}
}
@article{rink2014coupled,
	title={Coupled cell networks and their hidden symmetries},
	author={Rink, Bob and Sanders, Jan},
	journal={SIAM Journal on Mathematical Analysis},
	volume={46},
	number={2},
	pages={1577--1609},
	year={2014},
	publisher={SIAM}
}
@article{briand2003complete,
	title={A complete set of covariants of the four qubit system},
	author={Briand, Emmanuel and Luque, Jean-Gabriel and Thibon, Jean-Yves},
	journal={Journal of Physics A: Mathematical and General},
	volume={36},
	number={38},
	pages={9915},
	year={2003},
	publisher={IOP Publishing}
}
@article{stamatiou2007quantum,
	title={Quantum entanglement dependence on bifurcations and scars in non-autonomous systems. The case of quantum kicked top},
	author={Stamatiou, George and Ghikas, Demetris PK},
	journal={Physics Letters A},
	volume={368},
	number={3-4},
	pages={206--214},
	year={2007},
	publisher={Elsevier}
}
@article{lebovitz1998mathematical,
	title={The mathematical development of the classical ellipsoids},
	author={Lebovitz, Norman R},
	journal={International journal of engineering science},
	volume={36},
	number={12-14},
	pages={1407--1420},
	year={1998},
	publisher={Elsevier}
}
@article{fasso2001stability,
	title={Stability properties of the Riemann ellipsoids},
	author={Fass{\`o}, Francesco and Lewis, Debra},
	journal={Archive for rational mechanics and analysis},
	volume={158},
	number={4},
	pages={259--292},
	year={2001},
	publisher={Springer}
}
@book{nielsen2002quantum,
	title={Quantum computation and quantum information},
	author={Nielsen, Michael A and Chuang, Isaac},
	year={2002},
	publisher={AAPT}
}
@article{araujo2013classical,
	title={Classical bifurcation in a quadrupolar {NMR} system},
	author={Araujo-Ferreira, AG and Auccaise, R and Sarthour, RS and Oliveira, IS and Bonagamba, Tito Jos{\'e} and Roditi, I},
	journal={Physical Review A},
	volume={87},
	number={5},
	pages={053605},
	year={2013},
	publisher={APS}
}
@article{bhosale2017signatures,
	title={Signatures of bifurcation on quantum correlations: Case of the quantum kicked top},
	author={Bhosale, Udaysinh T and Santhanam, MS},
	journal={Physical Review E},
	volume={95},
	number={1},
	pages={012216},
	year={2017},
	publisher={APS}
}
@article{bogdanov2015study,
	title={The study of Lorenz and R{\"o}ssler strange attractors by means of quantum theory},
	author={Bogdanov, Yu I and Bogdanova, NA},
	journal={Laser Physics},
	volume={25},
	number={3},
	pages={035203},
	year={2015},
	publisher={IOP Publishing}
}
@article{feynman1982simulating,
  title={Simulating physics with computers},
  author={Feynman, Richard P},
  journal={International journal of theoretical physics},
  volume={21},
  number={6},
  pages={467--488},
  year={1982},
  publisher={Springer}
}
@inproceedings{bogdanov2019quantum,
	title={Quantum approach to the dynamical systems modeling},
	author={Bogdanov, Yu I and Bogdanova, NA and Fastovets, DV and Lukichev, VF},
	booktitle={International Conference on Micro-and Nano-Electronics 2018},
	volume={11022},
	pages={110222Q},
	year={2019},
	organization={International Society for Optics and Photonics}
}
@article{fasso2001stability,
	title={Stability properties of the {R}iemann ellipsoids},
	author={Fasso, Francesco and Lewis, Debra},
	journal={Archive for rational mechanics and analysis},
	volume={158},
	number={4},
	pages={259--292},
	year={2001},
	publisher={Springer}
}

@book{chandrasekhar1969ellipsoidal,
	title={Ellipsoidal figures of equilibrium},
	author={Chandrasekhar, Subrahmanyan},
	volume={9},
	year={1969},
	publisher={Yale University Press New Haven}
}

@book{golubitsky2003symmetry,
	title={The symmetry perspective: from equilibrium to chaos in phase space and physical space},
	author={Golubitsky, Martin and Stewart, Ian},
	volume={200},
	year={2003},
	publisher={Springer Science \& Business Media}
}



@article{rink2014coupled,
	title={Coupled cell networks and their hidden symmetries},
	author={Rink, Bob and Sanders, Jan},
	journal={SIAM Journal on Mathematical Analysis},
	volume={46},
	number={2},
	pages={1577--1609},
	year={2014},
	publisher={SIAM}
}


@article{nijholt2017projection,
	title={Projection blocks in homogeneous coupled cell networks},
	author={Nijholt, Eddie and Rink, Bob and Sanders, Jan},
	journal={Dynamical Systems},
	volume={32},
	number={1},
	pages={164--186},
	year={2017},
	publisher={Taylor \& Francis}
}

@article{mokhtari2019equivariant,
	title={Equivariant decomposition of polynomial vector fields},
	author={Mokhtari, Fahimeh and Sanders, Jan A},
	journal={arXiv preprint arXiv:1909.06955},
	year={2019}
}





@article{mokhtari2018representations,
	title={On the representations and $\mathbb{Z}/2$-equivariant normal form for solenoidal {H}opf-zero singularities},
	author={Mokhtari, Fahimeh},
	journal={Physica D: Nonlinear Phenomena},
	year={2018},
	publisher={Elsevier}
}


@article{gazor2013normal,
	title={Normal forms for {H}opf-Zero singularities with nonconservative nonlinear part},
	author={Gazor, Majid and Mokhtari, Fahimeh and Sanders, Jan A},
	journal={Journal of Differential Equations},
	volume={3},
	number={254},
	pages={1571--1581},
	year={2013}
}
@article{gazor2013volume,
	title={Volume-preserving normal forms of {H}opf-zero singularity},
	author={Gazor, Majid and Mokhtari, Fahimeh},
	journal={Nonlinearity},
	volume={26},
	number={10},
	pages={2809},
	year={2013},
	publisher={IOP Publishing}
}


@article{nijholt2016graph,
	title={Graph fibrations and symmetries of network dynamics},
	author={Nijholt, Eddie and Rink, Bob and Sanders, Jan},
	journal={Journal of Differential Equations},
	volume={261},
	number={9},
	pages={4861--4896},
	year={2016},
	publisher={Elsevier}
}


@book{HirschSmale1974,
	title={Differential equations, dynamical systems, and linear algebra},
	author={Hirsch, Morris W and Smale, Stephen},
	year={1974},
	publisher={Academic press}
}
@article{levelt1993semi,
	title={The semi-simple part of a matrix},
	author={Levelt, AHM},
	journal={Algoritmen In De Algebra (Aida), Nijmegen, August 1993},
	pages={83-86},
	year={1993},
	publisher={Citeseer}
}
@article{mokhtari2018versal,
	title={Versal Normal Form for Nonsemisimple Singularities},
	author={Mokhtari, Fahimeh and Sanders, Jan A.},
	journal={arXiv preprint arXiv:1808.02690},
	year={2018}
}


@article{gazormokhtari2014normal,
	title={Normal forms of {H}opf-zero singularity},
	author={Gazor, Majid and Mokhtari, Fahimeh},
	journal={Nonlinearity},
	volume={28},
	number={2},
	pages={311},
	year={2014},
	publisher={IOP Publishing}
}

@book{berhuy2010introduction,
	title={An introduction to Galois cohomology and its applications},
	author={Berhuy, Gr{\'e}gory},
	volume={377},
	year={2010},
	publisher={Cambridge University Press}
}
@Book{            MR0323842,
	author        = {Humphreys, J.},
	address       = {New York},
	year          = {1972},
	publisher     = {Springer-Verlag},
	title         = {Introduction to {L}ie {A}lgebras and {R}epresentation
	{T}heory}
}
@article {MR0161898,
	AUTHOR = {Gerstenhaber, M.},
	TITLE = {The cohomology structure of an associative ring},
	JOURNAL = {Ann. of Math. (2)},
	FJOURNAL = {Annals of Mathematics. Second Series},
	VOLUME = {78},
	YEAR = {1963},
	PAGES = {267--288},
	ISSN = {0003-486X},
	MRCLASS = {16.90 (18.00)},
	MRNUMBER = {MR0161898 (28 \#5102)},
	MRREVIEWER = {M. Auslander},
}
@misc{lewisfermat,
	title={Fermat User Guide},
	author={Lewis, R.H.}
}
@misc{lewis2008computer,
	title={Computer algebra system {F}ermat},
	author={Lewis, R.H.},
	year={2008}
}
@article{baez2014𝐺2,
	title={$\mathsf{G}_2$ and the rolling ball},
	author={Baez, J. and Huerta, J.},
	journal={Transactions of the American Mathematical Society},
	volume={366},
	number={10},
	pages={5257--5293},
	year={2014}
}
@article{Form00,
	title={{FORM} version 4.0},
	author={Kuipers, J. and Ueda, T. and Vermaseren, J.A.M. and Vollinga, J.},
	journal={Computer Physics Communications},
	volume={184},
	number={5},
	pages={1453--1467},
	year={2013},
	publisher={Elsevier}
}
@article{mailybaev2001transformation,
	title={Transformation to versal deformations of matrices},
	author={Mailybaev, A.A.},
	journal={Linear Algebra and its Applications},
	volume={337},
	number={1-3},
	pages={87--108},
	year={2001},
	publisher={Elsevier}
}
@article{koccak1984normal,
	title={Normal forms and versal deformations of linear Hamiltonian systems},
	author={Ko{\c{c}}ak, H.},
	journal={Journal of Differential Equations},
	volume={51},
	number={3},
	pages={359--407},
	year={1984},
	publisher={Elsevier}
}
@article{knibbeler2017higher,
	title={Higher-dimensional automorphic {L}ie algebras},
	author={Knibbeler, Vincent and Lombardo, Sara and Sanders, Jan A},
	journal={Foundations of Computational Mathematics},
	volume={17},
	number={4},
	pages={987--1035},
	year={2017},
	publisher={Springer}
}


@article{kulkarni1980sigurdur,
	title={Sigurdur {H}elgason, {D}ifferential geometry, {L}ie groups and symmetric spaces},
	author={Kulkarni, Ravi S and others},
	journal={Bulletin (New Series) of the American Mathematical Society},
	volume={2},
	number={3},
	pages={468--476},
	year={1980},
	publisher={American Mathematical Society}
}

@article{anderson2015non,
	title={Non-Isomorphic Real Simple {L}ie Algebras of the Same Complex Type and Character},
	author={Anderson, Ian M},
	year={2015}
}

@book{knapp2013lie,
	title={Lie groups beyond an introduction},
	author={Knapp, Anthony W},
	volume={140},
	year={2013},
	publisher={Springer Science \& Business Media}
}

@article{sanders1994versal,
	title={Versal normal form computations and representation theory},
	author={Sanders, J.A.},
	journal={Computer Algebra and Differential Equations’, Cambrige University Press, Cambrige},
	pages={185--210},
	year={1994}
}

@article{springer1966some,
	title={Some arithmetical results on semi-simple {L}ie algebras},
	author={Springer, Tonny A},
	journal={Publications Math{\'e}matiques de l'IH{\'E}S},
	volume={30},
	pages={115--141},
	year={1966}
}
@article{kostant1956principal,
	title={THE PRINCIPAL THREE-DIMENSIONAL SUBGROUP AND THE BETTI NUMBERS OF A COMPLEX SIMPLE LIE GROUP.},
	author={Kostant, Bertram},
	journal={Bull. Soc. Math. France},
	volume={84},
	pages={251--281},
	year={1956},
	publisher={JSTOR}
}
@article{kostant1963lie,
	title={Lie group representations on polynomial rings},
	author={Kostant, Bertram},
	journal={American Journal of Mathematics},
	volume={85},
	number={3},
	pages={327--404},
	year={1963},
	publisher={JSTOR}
}
@book {MR1890629,
	AUTHOR = {Bourbaki, Nicolas},
	TITLE = {Lie groups and {L}ie algebras. {C}hapters 4--6},
	SERIES = {Elements of Mathematics (Berlin)},
	NOTE = {Translated from the 1968 French original by Andrew Pressley},
	PUBLISHER = {Springer-Verlag},
	ADDRESS = {Berlin},
	YEAR = {2002},
	PAGES = {xii+300},
	ISBN = {3-540-42650-7},
	MRCLASS = {17-01 (00A05 20E42 20F55 22-01)},
	MRNUMBER = {1890629 (2003a:17001)},
}
@unpublished {KLS15c,
	AUTHOR = {Knibbeler, V. and Lombardo, S. and Sanders, J. A.},
	TITLE = {Automorphic {L}ie {A}lgebras and {C}ohomology of {R}oot {S}ystems},
	NOTE = {arXiv:1512.07020  [math-ph]},
	YEAR = {2015}
}





@book{golubitsky2003symmetry,
	title={The symmetry perspective: from equilibrium to chaos in phase space and physical space},
	author={Golubitsky, Martin and Stewart, Ian},
	volume={200},
	year={2003},
	publisher={Springer Science \& Business Media}
}


@article{rink2014coupled,
	title={Coupled cell networks and their hidden symmetries},
	author={Rink, Bob and Sanders, Jan},
	journal={SIAM Journal on Mathematical Analysis},
	volume={46},
	number={2},
	pages={1577--1609},
	year={2014},
	publisher={SIAM}
}


@article{nijholt2017projection,
	title={Projection blocks in homogeneous coupled cell networks},
	author={Nijholt, Eddie and Rink, Bob and Sanders, Jan},
	journal={Dynamical Systems},
	volume={32},
	number={1},
	pages={164--186},
	year={2017},
	publisher={Taylor \& Francis}
}






@article{gazor2013volume,
	title={Volume-preserving normal forms of {H}opf-zero singularity},
	author={Gazor, Majid and Mokhtari, Fahimeh},
	journal={Nonlinearity},
	volume={26},
	number={10},
	pages={2809},
	year={2013},
	publisher={IOP Publishing}
}

@article{nijholt2016graph,
	title={Graph fibrations and symmetries of network dynamics},
	author={Nijholt, Eddie and Rink, Bob and Sanders, Jan},
	journal={Journal of Differential Equations},
	volume={261},
	number={9},
	pages={4861--4896},
	year={2016},
	publisher={Elsevier}
}


@book{HirschSmale1974,
  title={Differential equations, dynamical systems, and linear algebra},
  author={Hirsch, Morris W and Smale, Stephen},
  year={1974},
  publisher={Academic press}
}
@article{levelt1993semi,
  title={The semi-simple part of a matrix},
  author={Levelt, AHM},
  journal={Algoritmen In De Algebra (Aida), Nijmegen, August 1993},
  pages={83-86},
  year={1993},
  publisher={Citeseer}
}
@article{mokhtari2018versal,
	title={Versal Normal Form for Nonsemisimple Singularities},
	author={Mokhtari, Fahimeh and Sanders, Jan A.},
	journal={arXiv preprint arXiv:1808.02690},
	year={2018}
}


@article{gazormokhtari2014normal,
	title={Normal forms of {H}opf-zero singularity},
	author={Gazor, Majid and Mokhtari, Fahimeh},
	journal={Nonlinearity},
	volume={28},
	number={2},
	pages={311},
	year={2014},
	publisher={IOP Publishing}
}

@book{berhuy2010introduction,
  title={An introduction to Galois cohomology and its applications},
  author={Berhuy, Gr{\'e}gory},
  volume={377},
  year={2010},
  publisher={Cambridge University Press}
}
@Book{            MR0323842,
  author        = {Humphreys, J.},
  address       = {New York},
  year          = {1972},
  publisher     = {Springer-Verlag},
  title         = {Introduction to {L}ie {A}lgebras and {R}epresentation
                  {T}heory}
}
@article {MR0161898,
AUTHOR = {Gerstenhaber, M.},
TITLE = {The cohomology structure of an associative ring},
JOURNAL = {Ann. of Math. (2)},
FJOURNAL = {Annals of Mathematics. Second Series},
VOLUME = {78},
YEAR = {1963},
PAGES = {267--288},
ISSN = {0003-486X},
MRCLASS = {16.90 (18.00)},
MRNUMBER = {MR0161898 (28 \#5102)},
MRREVIEWER = {M. Auslander},
}
@misc{lewisfermat,
  title={Fermat User Guide},
  author={Lewis, R.H.}
}
@misc{lewis2008computer,
  title={Computer algebra system {F}ermat},
  author={Lewis, R.H.},
  year={2008}
}
@article{baez2014𝐺2,
  title={$\mathsf{G}_2$ and the rolling ball},
  author={Baez, J. and Huerta, J.},
  journal={Transactions of the American Mathematical Society},
  volume={366},
  number={10},
  pages={5257--5293},
  year={2014}
}
@article{Form00,
  title={{FORM} version 4.0},
  author={Kuipers, J. and Ueda, T. and Vermaseren, J.A.M. and Vollinga, J.},
  journal={Computer Physics Communications},
  volume={184},
  number={5},
  pages={1453--1467},
  year={2013},
  publisher={Elsevier}
}
@article{mailybaev2001transformation,
  title={Transformation to versal deformations of matrices},
  author={Mailybaev, A.A.},
  journal={Linear Algebra and its Applications},
  volume={337},
  number={1-3},
  pages={87--108},
  year={2001},
  publisher={Elsevier}
}
@article{koccak1984normal,
  title={Normal forms and versal deformations of linear Hamiltonian systems},
  author={Ko{\c{c}}ak, H.},
  journal={Journal of Differential Equations},
  volume={51},
  number={3},
  pages={359--407},
  year={1984},
  publisher={Elsevier}
}
@article{knibbeler2017higher,
	title={Higher-dimensional automorphic {L}ie algebras},
	author={Knibbeler, Vincent and Lombardo, Sara and Sanders, Jan A},
	journal={Foundations of Computational Mathematics},
	volume={17},
	number={4},
	pages={987--1035},
	year={2017},
	publisher={Springer}
}


@article{kulkarni1980sigurdur,
	title={Sigurdur {H}elgason, {D}ifferential geometry, {L}ie groups and symmetric spaces},
	author={Kulkarni, Ravi S and others},
	journal={Bulletin (New Series) of the American Mathematical Society},
	volume={2},
	number={3},
	pages={468--476},
	year={1980},
	publisher={American Mathematical Society}
}

@article{anderson2015non,
	title={Non-Isomorphic Real Simple {L}ie Algebras of the Same Complex Type and Character},
	author={Anderson, Ian M},
	year={2015}
}

@book{knapp2013lie,
	title={Lie groups beyond an introduction},
	author={Knapp, Anthony W},
	volume={140},
	year={2013},
	publisher={Springer Science \& Business Media}
}

@article{sanders1994versal,
	title={Versal normal form computations and representation theory},
	author={Sanders, J.A.},
	journal={Computer Algebra and Differential Equations’, Cambrige University Press, Cambrige},
	pages={185--210},
	year={1994}
}

@article{springer1966some,
  title={Some arithmetical results on semi-simple {L}ie algebras},
  author={Springer, Tonny A},
  journal={Publications Math{\'e}matiques de l'IH{\'E}S},
  volume={30},
  pages={115--141},
  year={1966}
}
@article{kostant1956principal,
  title={THE PRINCIPAL THREE-DIMENSIONAL SUBGROUP AND THE BETTI NUMBERS OF A COMPLEX SIMPLE LIE GROUP.},
  author={Kostant, Bertram},
  journal={Bull. Soc. Math. France},
  volume={84},
  pages={251--281},
  year={1956},
  publisher={JSTOR}
}
@article{kostant1963lie,
  title={Lie group representations on polynomial rings},
  author={Kostant, Bertram},
  journal={American Journal of Mathematics},
  volume={85},
  number={3},
  pages={327--404},
  year={1963},
  publisher={JSTOR}
}
@book {MR1890629,
    AUTHOR = {Bourbaki, Nicolas},
     TITLE = {Lie groups and {L}ie algebras. {C}hapters 4--6},
    SERIES = {Elements of Mathematics (Berlin)},
      NOTE = {Translated from the 1968 French original by Andrew Pressley},
 PUBLISHER = {Springer-Verlag},
   ADDRESS = {Berlin},
      YEAR = {2002},
     PAGES = {xii+300},
      ISBN = {3-540-42650-7},
   MRCLASS = {17-01 (00A05 20E42 20F55 22-01)},
  MRNUMBER = {1890629 (2003a:17001)},
}
@unpublished {KLS15c,
AUTHOR = {Knibbeler, V. and Lombardo, S. and Sanders, J. A.},
TITLE = {Automorphic {L}ie {A}lgebras and {C}ohomology of {R}oot {S}ystems},
NOTE = {arXiv:1512.07020  [math-ph]},
YEAR = {2015}
}


